Dynamic Information Sub-Selection for Decision Support

We introduce Dynamic Information Sub-Selection (DISS), a novel framework of AI assistance designed to enhance the performance of black-box decision-makers by tailoring their information processing on a per-instance basis. Blackbox decision-makers (e.g., humans or real-time systems) often face challenges in processing all possible information at hand (e.g., due to cognitive biases or resource constraints), which can degrade decision efficacy. DISS addresses these challenges through policies that dynamically select the most effective features and options to forward to the black-box decision-maker for prediction. We develop a scalable frequentist data acquisition strategy and a decision-maker mimicking technique for enhanced budget efficiency. We explore several impactful applications of DISS, including biased decision-maker support, expert assignment optimization, large language model decision support, and interpretability. Empirical validation of our proposed DISS methodology shows superior performance to state-of-the-art methods across various applications.

==> sections/old_experiments.tex <==
In this section, we first conduct an extensive set of experiments to demonstrate our proposed Frequentist Thompson Sampling (FTS) and Mimic-Structured Regression approaches can outperform or on par with baseline methods under different environments (different class of experts). Since one of our target application is to provide decision support to human experts, our second set of experiments are devised to simulate cognitive biases experienced by human experts. Another way that DISS can be used to facilitate human decision maker is to provide personalized subset of features models; in this set of experiment, we introduce a penalty term to encourage the policy to use the smallest subset of features to make inference while maintaining task performance. Lastly, recent development in generative modeling allows humans using large language models to find answers to questions; in this set of experiment, we explore the possibility of using DISS policy to select not only a subset of features for any given instances but also select appropriate prompt style.

In all experiment except the large language model ones, we used publicly available skin segmentation \citep{bhat-2009}, Statlog (Shuttle) \citep{-}, and SUSY \citep{whit-2014} datasets from UCI machine learning repository as the underlying task represented by the environment \todo{supply a table in appendix that list each dataset's number of instances and number of features}; for each task, we use two types of classifiers -- Nadaraya-Watson kernel regression (NWC) and personalized k-nearest neighbors logistic regression (KNNLRC) -- to perform the subset feature classification; in total, this creates 6 environments. We use negative cross-entropy loss between subset feature classifier output and the ground truth label as the reward signal which our DISS policy aims to maximize. We compare our proposed frequentist continuous multitask Thompson sampling (FCMTS) and mimic structured regression (Mimic) against Modiste \citep{Bhatt2023} and random strategy. Note that the original Modiste paper assumed the reward to be bounded and discrete; yet, our reward is continuous and unbounded. As workaround, we make two attempts: the first approach -- Modiste KNN -- follows the original Modiste paper, but we initialize previously unseen reward to be the minimum reward stored in the replay buffer; the second approach -- Modiste UKNN -- concatenates feature mask to context and performs k-nearest neighbor regression in this space. \todo{add corresponding appendix} In addition, we used continuous multitask Thompson sampling (CMTS) \citep{Char2019} with Gaussian Process regressor on the skin NWC environment as skin segmentation dataset only has three features.

% \subsection{Synthetic Expert Experiments}
% The learning curve of our proposed method and each baseline for each environment is presented in \autoref{fig:human_decision_rlc}. We first note that our proposed mimic-structure regressor outperforms all the other baseline across the board, which validates our intuition about taking advantages of the known reward structure. Second, we observe that Modiste KNN are unstable in environments that have higher dimensional contexts; we conjecture the reason is twofold: first, the action space grows combinatorially as number of features increases, which makes gathering enough samples for each action more and more difficult; second, since our reward is continuous and unbounded, we don't have an easy way of initializing reward estimates for those not-yet-pulled arms to a fixed value that entails maximum entropy, e.g. 0.5 for a zero-one reward environment.\todo{perhaps fallback to each environment has its own plot so that i can autoref to subfigures} Third, CMTS in Skin NWC experiment did not finish within the given time budget as the parameters to Gaussian Process is updated through gradient descent after the policy makes an acquisition; similarly, Modiste UKNN did not finish in both environment that uses SUSY dataset due to KNN computations eventually run out of memory; both cases suggested that ``distance-based'' score estimators might not be suitable for our DISS contextual bandit setting where dimensionality is a concern.

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{strategy/basic.jpg}
%     \caption{Reward learning curves.}
%     \label{fig:human_decision_rlc}
% \end{figure}

\subsection{Biased Synthetic Expert Setting}
\label{biased_synth_exp}

\subsubsection{Bias Implementation}
Motivated by the target application of providing decision support to human experts, we have devised a set of experiments featuring a synthetic decision maker exhibiting various forms of simulated cognitive bias:
\paragraph{Cognitive Overload.} While more information may lead to better quality predictions in theory, human experts are hampered in practice by the limited ability of their working memory to hold multiple simultaneous pieces of information. When these limits are reached, the expert is likely to experience "cognitive overload," making it difficult to predict accurately and with confidence. \citep{iskander_burnout_2018}

We simulate the effects of cognitive overload by applying a temperature-controlled softmax activation function to the output logits obtained from our synthetic expert:
\begin{equation}
  \text{softmax}(\mathbf{\hat{y}}, \mathbf{b})_i = \frac{\exp{(\frac{\hat{y}_i}{T(\mathbf{b})}})}{\sum_{j}^{\text{nclass}}\exp{(\frac{\hat{y}_j}{T(\mathbf{b}}})}
  \label{eq:softmax_temp}
\end{equation}

where $T(\mathbf{b})$ is a temperature function whose value increases as more features are observed in $\mathbf{b}$. (Specifically, we set $T(\mathbf{b})$ to be proportional to the Euclidean norm of $\mathbf{b}$.)

In order to provide effective decision support to this type of expert, we expect our policy to learn a small but efficient feature subset that allows accurate prediction while incurring minimal uncertainty penalties.

\paragraph{Risk Aversion.} When tasked with making certain types of binary decisions, experts may be reluctant to risk reporting false negative results; this phenomenon has been previously observed in medical settings where the cost of a missed diagnosis could be life-threatening \citep{sorum_risk_2003}.

To simulate risk aversion, we combine the expert's prediction with a 100\% positive prediction $([0, 1])$, weighted by a bias strength parameter $\alpha$:

\[ \hat{y}_{\text{averse}} = (1-\alpha) \cdot \hat{y}+ (\alpha) \cdot [0, 1] \]

To successfully support this expert's decision making, we expect our policy to select features that increase the expert's confidence when predicting negative examples. For example, if the policy function believes the current instance is negative, features that would skew the prediction in the positive direction may be omitted to avoid triggering the expert's bias.

\paragraph{Statistical Discrimination.} Rather than view a data profile holistically, experts may allocate undue attention towards irrelevant or prejudicial factors. The latter is a pervasive problem in the medical field, where racial and gender biases are known to lead to discrepancies in treatment recommendations. \citep{chen_racial_2001, schulman_effect_1999}

Similar to the implementation of risk aversion, we model statistical discrimination in prediction by computing a convex combination between the expert's original prediction and a biased prediction. In this case, the biased prediction comes from a univariate classification model $g(x_j)$ trained on the $j^{th}$ feature column of the data used to train the main expert. We refer to feature $j$ as the "poison feature." If the poison feature is observed in $\mathbf{b}$, the expert's original prediction will be modified as

\[ \hat{y}_{\text{poison}} = (1-\alpha) \cdot \hat{y}+ (\alpha) \cdot g(x_j) \]

Otherwise, the prediction will be unchanged.

To avoid the effects of the statistical discrimination bias, we expect our method to learn a policy that avoids including the poison feature in the subsets presented to the expert.
\begin{figure}[h]
\centering
    \includegraphics[width=\linewidth]{images/bias/poison_conf_v2.jpg}
    \caption{Learning curves for DISS compared to a baseline selection approach (Modiste) on the \textbf{skin}, \textbf{space}, and \textbf{susy} UCI datasets.}
\end{figure}

\subsection{Multi-Expert Setting}

In this experimental setting, we consider a scenario where multiple decision makers are available to the policy, but only one can be queried for cost reasons. Thus, in addition to selecting a subset of features to display, the policy must also select which decision maker should predict on a given data point.

In a real world setting, decision makers may have varying expertise on different sub-regions of a data space. In our synthetic expert experiments, we simulate this property by separating our data into clusters and providing each expert with a single cluster as the support for their knowledge base. For our experimental trials, we performed K-Means clustering on each dataset with $k=4$, resulting in $4$ distinct experts for our policy to choose from. Unlike the biased synthetic expert setting in \autoref{biased_synth_exp}, in these experiments the synthetic experts were not modified with any additional source of limitation or bias; only the source of the models' training data differed between experts.
\begin{figure}[h]
\centering
    \includegraphics[width=\textwidth]{images/multi/multi_conf_v2.jpg}
    \caption{Learning curves in the multi-expert setting for DISS and Modiste.}
\end{figure}

\subsection{Visualization and Interpretability}\label{sec:exp_interpretability}
In this experiment, we attempted to minimize the subset of features selected to reduce cognitive overload and used our proposed new class of interpretable model KNNLRC as proposed in \autoref{sec:applications} to perform the classification.

Recall the reward $r$ define in \autoref{eq:base_reward} for our synthetic expert experiment is the negative cross-entropy between subset feature classifier output probability and the ground truth label. In this experiment, we introduce a penalty term that subtract number of features selected weighted by a hyperparameter $\beta$ encouraging policy to use a more compact subset of features. The new reward for this experiment is therefore defined as
\begin{equation}
    r_{\text{new}} = r - \beta \left\lVert b \right\rVert _{1}
\end{equation}

In \autoref{fig:beta_sweep_curves}, we first demonstrate our proposed method -- Mimic and FCMTS -- performed better compare to all the other baseline methods across different environments; in particular, Mimic approach typically reaches its top performance faster than FCMTS even though both Mimic and FCMTS could eventually converge to the same reward, which verifies our intuition regarding taking advantages of our prior knowledge to the reward signal and therefore has better sample efficiency than its counterpart. It is also observed that the learning curve is visually smoother as $\beta$ increases; we conjecture that the strength of the penalty term ``eliminated'' some actions in the action space that could reach the same negative cross-entropy but uses more features, which resulted in the policy has fewer options to consider during the learning phase.
\todo{susy is just a placeholder here. Waiting for its result to come out}
\begin{figure}[h]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/curve/skin_alpha_sweep.jpg}
            % \caption{}
            % \label{fig:skin_knnlrc_beta_sweep_curves}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/curve/space_alpha_sweep.jpg}
            % \caption{}
            % \label{fig:space_knnlrc_beta_sweep_curves}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/curve/susy_alpha_sweep.jpg}
            % \caption{}
            % \label{fig:susy_knnlrc_beta_sweep_curves}
        \end{subfigure}
    \end{subfigure}
    \caption{DISS learning curve in KNNLRC under different penalty weight $\beta$. Black dots represents task performance using DISS policy selected subset of features, whereas red stars represent task performance using randomly selected subset of features.}
    \label{fig:beta_sweep_curves}
\end{figure}

We sweep over the $\beta$ term to test the effectiveness of the proposed penalty term. First, it is observed that the number of features selected drastically decreases as the penalty strength parameter $\beta$ increases from first row of \autoref{fig:beta_nfeats_sweep}. Second, the black dots in the last two rows of \autoref{fig:beta_nfeats_sweep} suggest task performances remain more or less remain constant as average number of selected features decrease.\footnote{In \autoref{fig:beta_nfeats_sweep}, number of features selected are not integer and the reason is that it's the number of features selected under expectation.} Third, to test if our selected features are actually informative, we measure task performances using randomly selected subset of features and are represented by the red dots in \autoref{fig:beta_nfeats_sweep}.\footnote{When we select same number of features at random, whether a feature will be included in the subset is a Bernoulli trial with probability $p=\frac{\text{number selected}}{d}$.} It can be seen that features selected with DISS (black dots) yield better performance than that of randomly selected ones, which demonstrates our DISS policy is indeed selecting informative subset of features while keeping the subset as compact as possible.
\todo{susy is just a placeholder here. Waiting for its result to come out}
\begin{figure}
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/beta_nfeats/skin_nfeats.jpg}
            \caption{}
            % \label{fig:skin_knnlrc_beta_sweep_curves}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/beta_nfeats/space_nfeats.jpg}
            \caption{}
            % \label{fig:space_knnlrc_beta_sweep_curves}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/beta_nfeats/susy_nfeats.jpg}
            \caption{}
            % \label{fig:susy_knnlrc_beta_sweep_curves}
        \end{subfigure}
    \end{subfigure}
    \caption{DISS learning curve in KNNLRC under different penalty weight $\beta$.}
    \label{fig:beta_nfeats_sweep}
\end{figure}

Next, we demonstrate the capability of our proposed KNNLRC model for two-dimensional cases. We recognized that it is possible for the DISS policy to select a subset of features that has more than three elements and humans are only be able to visualize up to three-dimensional data. However, as shown in \autoref{fig:beta_nfeats_sweep}, one can limit the number of features selected through controlling penalty coefficient $\beta$ without significantly impacting task performance. We argue that presenting a reasonable subset of features directly to humans is already acceptable in certain applications; for example, a doctor could already comprehend from a list of patients with similar lab result readings without relying on visualization. In \autoref{fig:personalized_model_space_showcase}, we plot the query instance in red star along with the nearest neighbors in the training set of the query with class label 0 and 1 in tan and blue dots, respectively. In \autoref{fig:space_knnlrc_purity}, the KNNLRC expert is able to make correct inference using either DISS selected features or randomly selected features; yet, it can be observed that the nearest neighbors in the DISS selected two features has higher purity, i.e. most neighbors have the same class label as the true ones, compare to that of in the randomly selected two features. On the other hand, there are also cases where the randomly selected two features would cause the KNNLRC to misclassify the query as shown in \autoref{fig:space_knnlrc_wrong}.
\todo{susy is still a pending case}
\begin{figure}
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/model/space/structure/conf_91.jpg}
            \caption{}
            \label{fig:space_knnlrc_purity}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/model/space/structure/conf_21.jpg}
            \caption{}
            \label{fig:space_knnlrc_wrong}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{personalized/model/space/structure/conf_91.jpg}
            \caption{}
            \label{fig:susy_knnlrc_pending}
        \end{subfigure}
    \end{subfigure}
    \caption{Two-dimensional visualization of the proposed KNNLRC model with subset of features selected with DISS policy versus that of chosen randomly.}
    \label{fig:personalized_model_space_showcase}
\end{figure}

\subsection{Large Language Model Setting}\label{sec:llm_setting}
LLMs have been proved to be effective in distilling common-sense knowledge about various domains, making them to ideal candidates mimic the black-box decision maker. By leveraging this behaviour of LLMs, we can create a system that captures complex decision making process. In this section, we evaluate the effectiveness of our feature selection method using the different combinations of acquisition strategies that we propose in section \autoref{sec:subsec2.2} across two datasets, Diabetes dataset \citep{diabetes} and California Housing Dataset \citep{housing}. We use to \texttt{Meta-Llama-3.1-8B-Instruct-Turbo} model for the LLM as it achieves strong performance on a number of benchmarks \citep{dubey2024llama3herdmodels}. We provide the prompt format which is a combination of components which are selected by our trained policy function $<Preamble> \wedge <feature> \wedge <output style>$. Our experimental methodoloy employes two types of regressors for each task: vanilla regressors and Mimic-based regressors to estimate rewards and perform feature subset selection. We use negative cross-entropy loss between LLM output classifier and the ground truth label as the reward signal which out DISS policy aims to maximize. We compare our proposed Frequentist Continous Multitask Thompson Sampling (FCMTS) and mimic structured regression (Mimic) against random strategy (Random). It can be noticed that our methods, FCMTS and Mimic, perform better than the random acquisition strategy.

To illustrate our method on LLMs, we present a compartivie analysis of two examples. compare two examples, which are also graphically shown in \todo{reference figure} demonstrating the feature selections using our methods vs random selection of features for the same instances in terms of outputs from LLMs. This side-by-side comparision offers insights into how our approach improves the quality and relevance of LLM outputs in decision support contexts. More such examples can be found in the Appendix \todo{cite appendix}
\todo{please change the figsize in your plotting yaml.}
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/llm_figures/llm.png}
    \caption{DISS learning curves in the LLM setting. Orange represents the reward obtained using mimic structure based policy. Green dotted represented FCTMS and dashed dot represents random selection.}
    \label{fig:llm-result}
\end{figure}

\paragraph{Mimic based selection of features}
\begin{mdframed}
    \texttt{
        \item \textbf{Prompt:} You are an AI model trained to predict whether a patient has diabetes based on certain medical features. Your task is to analyze the given provided features and provide a prediction.
        \item \textbf{Some important notes:} Not all features may be provided for every prediction. Please interpret these as best as you can and state the explanation behind your prediction.
        \item You will be given the following features for a patient: <Gender of the patient, Age of the patient (in years), Whether the patient has hypertension (0 for No, 1 for Yes), Whether the patient has heart disease (0 for No, 1 for Yes), Patient's smoking history, Body Mass Index (weight in kg / (height in m$^2$)), HbA1c level in blood (glycated hemoglobin), Blood glucose level (mg/dL)>
        \item Strictly follow this <output format>
        \item 1. \textbf{Prediction:} State whether the patient is likely to have diabetes "Positive" or "Negative", and mention how confident you are [Low, Moderate, High]
        \item 2. \textbf{Confidence:} Express your confidence as a probability strictly in this <format> the scores should range from 0 to 1.
        \item 3. \textbf{Provide explanation for your predictions}
        Please provide your prediction for the following <Patient has hypertension, Patient's smoking history is True, HbA1c level is 6.09, and the blood glucose level is 160.0>
    }
\end{mdframed}
% \newline
Here's the LLM output:
\tiny
\begin{mdframed}
    \texttt{
        1. \textbf{Prediction:} Positive, High
        2. \textbf{Confidence:} 0.95
        3. \textbf{Explanation:}
        \item The patient has hypertension (1.0), which is a known risk factor for diabetes.
        \item The patient has a smoking history (1.0), which is also a risk factor for diabetes.
        \item The patient's HbA1c level (6.099999904632568) is above the normal range (typically < 5.7\%), indicating potential glucose regulation issues.
        \item The patient's blood glucose level (160.0 mg/dL) is higher than the normal range (typically < 100 mg/dL), further indicating potential glucose regulation issues.
        \item Given these factors, the patient's likelihood of having diabetes is high. However, I would like to note that a crucial piece of information is missing - the patient's age. Age is an important factor in diabetes prediction, and without it, my confidence in the prediction is slightly lower than it could be. Nevertheless, based on the available data, I am confident that the patient is likely to have diabetes.
    }
\end{mdframed}
\normalsize
\paragraph{Random statergy of selecting features}
\todo{the prompt has similar structure with mimic based selection of features; would it be possible to just highlight the difference instead of repeatign the same thing over and over?}
\begin{mdframed}
    \texttt{
        \item \textbf{Prompt:} You are an AI model trained to predict whether a patient has diabetes based on certain medical features. Your task is to analyze the given provided features and provide a prediction.
        \item \textbf{Some important notes:} Not all features may be provided for every prediction. Please interpret these as best as you can and state the explanation behind your prediction.
        \item You will be given the following features for a patient: <Gender of the patient, Age of the patient (in years), Whether the patient has hypertension (0 for No, 1 for Yes), Whether the patient has heart disease (0 for No, 1 for Yes), Patient's smoking history, Body Mass Index (weight in kg / (height in m$^2$)), HbA1c level in blood (glycated hemoglobin), Blood glucose level (mg/dL)>
        \item Strictly follow this <output format>
        \item 1. \textbf{Prediction:} State whether the patient is likely to have diabetes "Positive" or "Negative", and mention how confident you are [Low, Moderate, High]
        \item 2. \textbf{Confidence:} Express your confidence as a probability strictly in this <format> the scores should range from 0 to 1.
        \item 3. \textbf{Provide explanation for your predictions}
        Please provide your prediction for the following <HbA1c level is 6.09, and the blood glucose level is 160.0>
    } \newline
\end{mdframed}
Here's the LLM output:
\begin{mdframed}
    \texttt{
        1. \textbf{Prediction:} Negative, High
        2. \textbf{Confidence:} 0.05
        3. \textbf{Explanation:}
        \item The given data includes HbA1c level and blood glucose level, which are crucial for predicting diabetes. The HbA1c level is 6.099999904632568, which is higher than the normal range (typically < 5.7). The blood glucose level is 158.0 mg/dL, which is higher than the normal range (typically < 100 mg/dL). These values indicate that the patient may be at risk for diabetes.
        \item However, the data is missing some crucial features such as age, hypertension, heart disease, and bmi, which can also influence the prediction. Without these features, the prediction is based on the available data and may not be as accurate.
        \item Considering the available data, the patient's HbA1c level and blood glucose level suggest a low risk for diabetes.
    }
\end{mdframed}


==> sections/old_methods.tex <==
\subsection{Problem Setting}
Below we formally introduce our task. Throughout, we use a running example of clinical decision making for illustrative purposes.

\paragraph{Decision Maker}
We seek to maximize rewards for the decisions of a black-box decision-maker $M$, that ingests: 1) arbitrary subsets of available information on an instance $x$, and 2) additional options $o$ (both of which will impact $M$’s outputs). For example, a clinician may ingest a given subset of patient features in a visual display style specified by $o$. For notational simplicity, we take $x \in \mathbb{R}^d$. For each instance, we consider $M$'s decision space to be binary for simplicity $\hat{y}\in \{0,1\}$ (e.g., whether or not to employ a treatment). In this case, the black-box decision-maker $M$ makes decisions based on subsets of features, $b \in \{0, 1\}^d$, and additional options $o \in \mathbb{O}$, as $M(x \odot b, b, o)$, where $\odot$ denotes the Hadamard product. We consider the output space of $M$ to be $[0, 1] \times \mathbb{M}$, the tuple of $M$'s probability of selecting action $\hat{y}=1$, along with any additional meta-data $m\in \mathbb{M}$ that is relevant for assessing decision quality. For example, a clinician outputs a confidence of their decision (probability of $\hat{y}=1$), along with a recorded time taken to decision (the meta-data $m$).

\paragraph{DISS Policy and Criterion}
We consider a reward based on the the output of the decision maker and the ground truth optimal decision $y$ for an instance $x$, $r(y, M(x \odot b, b, o)$.
We wish to learn a policy $\pi: \mathbb{R}^d \mapsto  \{0, 1\}^d \times \mathbb{O}$, that maximizes this reward over a data distribution of instances, $\mathcal{D}$. That is, we want to learn
\[\mathrm{argmax}_{\pi \in \Pi} \mathbb{E}_{(x,y)\sim \mathcal{D}}[r(y, M(x \odot \pi_b(x) , \pi_b(x), \pi_o(x))]. \]
To train the policy, we assume that we have a standard supervised dataset $D = \{(x^{(i)}, y^{(i)})\}_{i=1}^n$. Note, however, that $D$ does not contain any information about the decision-making of $M$, which the policy must consider. For many real-world applications, we will be limited on the number of calls that can be made to the black-box decision-maker $M$ during training. Thus, we consider a fixed-budget of $K$ queries to $M$ that is possible to optimized (TODO eqref above). [[TODO: y'all should clean this up.]]

\subsection{Frequentist Multi-Task Optimization}

\paragraph{Avoiding Gaussian Processes}
Our primary approach to solving the DISS problem draws inspiration from Continuous Multi-Task Thompson Sampling \citep{Char2019}. As previously mentioned, this algorithm relies on a Gaussian Process to produce randomly varying estimators $f \sim GP(\mu, \sigma)$, which has the drawback of scaling poorly in high dimensions. To address this issue, we instead train an ensemble $F$ consisting of $m$ diverse reward predictors and sample $f \sim F$ by randomly selecting one member of the ensemble with uniform probability $\frac{1}{m}$. Hence, we create a discrete random distribution over estimator functions as a substitute for the posterior distribution created by the mean and covariance functions of the GP.

\paragraph{Bootstrapped Ensembles of Predictors}
We create the ensemble $F$ in a bootstrapped manner by training individual regressors on overlapping random subsets of the training data, where each context $\times$ action $\times$ reward tuple $(x, b, o, r)$ appears in a given training subset with probability $p=\gamma$. [[TODO: more rigorous detail on the statistical implications of this process?]]

\subsection{Augmented Estimator Training}
\paragraph{Data Availability Assumption} In a real-world setting, ground-truth reward values obtained by querying an expert are likely to be limited in quantity due to cost. However, more data may be available in the form of a standard supervised dataset. We propose a way to leverage this additional resource by deconstructing the process of estimating the reward obtained by the expert.
\paragraph{Reward Estimation Process}
Consider a reward function \[r(y, M(x \odot \pi_b(x) , \pi_b(x), \pi_o(x)))\]
Implicitly, the process of obtaining an estimated reward $\hat{r}(x, b)$ involves estimating
\[p(y|x)\]
as well as
\[p(\hat{y}|M, x, b, o)\]
where $\hat{y} = \mathrm{argmax}\  M(x \odot \pi_b(x) , \pi_b(x), \pi_o(x))$. A vanilla regression approach to reward estimation can be thought of as estimating both of these quantities, along with the correct evaluation of $r$ applied to the resulting values. We propose to approach this estimation in a more direct manner that also leverages additional supervised data by creating a split-function structured regressor.
\paragraph{Structured Regression Approach}
The first component of our structured regression model is a standard supervised classifier $\Tilde{f}$ that directly models $p(y|x)$ in order to produce an estimate $\Tilde{y}$ of the ground truth label associated with the given example. $\Tilde{f}$ can be trained on all available supervised data for the target problem (as opposed to the limited set of expert queries.)

The structured model also contains a "mimic" model $\Tilde{M}$ whose purpose is to imitate the behavior of the expert, i.e. modeling $p(\hat{y}|M, x, b, o)$ as precisely as possible. $\Tilde{M}$ is trained on the set of expert queries, using the prediction probabilities $M(x \odot \pi_b(x) , \pi_b(x), \pi_o(x))$ provided by the expert as targets.




==> sections/old_related.tex <==
\subsection{Data-Driven Adaptable Displays}
Our research aims to develop techniques for intelligently filtering the information presented to an expert in order to achieve better decision making outcomes. While this particular framing of the aforementioned objective is unexplored, the broader problem of providing decision support via adaptive interfaces has been studied in the context of human-computer interaction (HCI). \citep{wang_adaptive_2024} reviewed existing literature relating to adaptive user interfaces for long-term health patients and observed that predictive algorithms (e.g. reinforcement learning, Monte Carlo tree search) were used somewhat commonly as an adaptation strategy.  \citep{chan_designing_2022} contribute to this area by investigating optimization-driven design approaches in HCI, particularly focusing on Multi-Objective Bayesian Optimization (MOBO) for exploring design spaces in interaction techniques. Their study found that optimization-driven design improved outcomes in terms of efficiency and accuracy. \citep{buçinca_offline_2024} explore the potential of offline reinforcement learning to optimize human-AI interaction, and demonstrate success in enhancing the accuracy of human decision making with AI support. \citep{salima_interface_2023} extend the exploration of adaptive decision support by proposing a framework for context-aware human-machine interfaces, emphasizing the integration of data pertaining to the user's cognitive state as well as the state of the machine and its environment. Their approach connects decision support directly to interface adaptation, providing flexibility in how information is presented based on real-time conditions.

Many research efforts (including ours) frame the task of optimizing decision support systems as a multi-armed bandit problem. \citep{lomas_bandit_2016} employed multi-armed bandits to optimize the experience of an online educational game by selecting among several possible variants. \citep{nikolov_interface_2019} propose a contextual bandit approach to solving the interface selection problem in Industrial IoT networks; their modified version of the Linear Upper Confidence Bound (LinUCB) algorithm optimizes wireless network selection by obtaining data rate estimates from channel quality parameters.

\subsection{Contextual Bandit Problems}
Multi-armed bandit problem \citep{Lattimore2020} is a classical online learning framework stated as follows: given $K$ arms (or actions) with each associated with a fixed but unknown reward probability distribution, an agent selects an action based on a policy then receives a reward sampled from the reward probability distribution associated with the chosen action. The goal of a bandit algorithm is to let the player learn the optimal policy within horizon $N$, i.e. within $N$ interactions with the environment. One particular variant of multi-armed bandit problem is contextual multi-armed bandit problem, or simply contextual bandit; at each round, the agent gets to observe an additional feature vector termed context and use this additional information to choose an action accordingly.

We formulate DISS as a contextual multi-armed bandit problem, where each instance $x \in \mathbb{R}^d$ is considered as the context, all the possible combination of $d$ features is considered as the action space, and the environment takes the selected subset of features from the context to make inference and returns a reward that signals the quality of the selection. Note that the cardinality of the action space $\left\lvert \mathcal{A} \right\rvert = \sum_{i=1}^{d} \binom{d}{i} $ grows combinatorially as number of features in context increases, which makes prior works such as Modiste \citep{Bhatt2023} that maintains $\left\lvert \mathcal{A} \right\rvert$ reward estimators for each action infeasible in high-dimensional setting. In fact, the term combinatorial multi-armed bandit refers to the class of bandit problem with combinatorial size action space \citep{Gai2012,Chen2013,Chen2016,Wang2018}; actions in the action space can be classified as either a base arm (action) or a super arm (action) in combinatorial multi-armed bandit problem. In our DISS terminology, actions that select only one feature from the given instance are base actions and those that select two or more features are super actions.

Prior works have proposed applying combinatorial multi-armed bandit to solve online feature acquisition \citep{Durand2014,Bouneffouf2017}. Two points are worth mentioning. First, one fundamental difference between online feature selection \citep{Wang2013,Durand2014} and our proposed DISS is that the former aims at using bandit to identify the optimal subset of features that could be used to train a classifier (expert) using most relevant features, whereas our DISS aims at learning a policy to provide a subset of features that could enable our downstream expert (potentially human expert) to achieve optimal inference performance; in other words, online feature selection involves training the expert whereas we assume the expert is a fixed function that we can only make query with. Second, works in combinatorial multi-armed bandit often make assumption about the relation between super action reward and base action reward, i.e. super action reward can be written in terms of base action reward, such as contextual bandit with restricted context proposed by \citeauthor{Bouneffouf2017} that defines the reward of super actions as the sum of the reward acquired from individually taking each base action in the currently selected super action, which is not suitable in our application. In a lot of cases, certain subset of features must be presented at the same time to make sense for the downstream expert but not when presented individually. \todo{think of an example; i don't know if there is a disease where a doctor can only make diagnosis based on certain subset of test.}

In this work, we borrow the idea from Multi-Task Thompson Sampling (MTS) \citep{Char2019} originally proposed to solve nuclear fusion problem. The MTS method utilizes one Gaussian Process (GP) instance to capture the relation between reward and context-action pair and the MTS acts optimally with respect to samples drawn from the GP posterior. That is, at every round, a sample of estimated reward function is drawn from the GP instance and the sample is used as if it were the ground truth reward. We concatenate the context with the selected feature mask as input to the reward estimator, which alleviates the need to maintain an estimator for each action. As GP does not well with big-data \citep{Murphy2022}, we replace GP with bootstrap of ``light models'' that are quick to fit and fast to run inference.

\subsection{Prompt Engineering LLMs}
Prompting is an efficient method of adapting Language Models to new tasks not seen during training without needing expensive re-training \citep{Radford2019LanguageMA}. In a typical prompting setup, a model autoregressively completes the next output tokens conditioned on the provided prompt and optionally additional information, such as examples from the query dataset \citep{few-shot}. The proliferation of different prompting styles such as in-context learning \cite{few-shot}, instruction following \cite{wei2022chain}, chain-of-thought prompting \cite{wei2022finetuned} and prompt-tuning \cite{lester-etal-2021-power} lacks theory of the underlying mechanisms and the effectiveness of these methods remains largely empirical with prompt choices based on average results on the validation set \cite{Burnell2023-sn}, which doesn't account for the variance in performance in real-life scenarios. Recent works also show that the LLM outputs are sensitive to the prompting style, position of information in the prompt, and the length of the prompt \citep{liu-etal-2024-lost}, \citep{Zhao2021CalibrateBU}, hence requiring the need for a logical breakdown of the query into smaller functions and conjoining them with human feedback or external systems guiding them into a meaningful prompt to generate meaningful outcomes from the LLM. \newline
\textbf{LLMs for feature selection:}
Previous work such as \citep{Choi2022LMPriorsPL} developed techniques for predicting with suitable language-model based priors, which incorporated task-specific priors to encourage downstream model outputs. \cite{zollo2023prompt} introduces an approach to select prompts from a static set based on rigorous upper bounds to avoid unacceptable outcomes generated by the LLM. However, this work is limited to the expertise of the prompt designer to create a fixed set of candidate prompts. We select each prompt component using a data-driven external policy function, making it more customized to each domain in order to maximize the efficacy of the decision-maker. 
\citep{jeong2024llmselectfeatureselectionlarge}
Administrative tasks, especially in hospitals and Electronic Healthcare Record Systems (EHR), are contributing to clinician burnout \citep{Adler-Milstein2020-fs}.  This same study shows a percentage of LLM answers to patients had safety errors, and some advice given could also be fatal. Previous studies assessed the quality of LLMs to clinical questions. However, the effectiveness of LLMs in improving efficiency and cognitive overload is not yet proven.
